Trace and Stable Failures Semantics for CSP-Agda

CSP-Agda is a library, which formalises the process algebra CSP in the interactive theorem prover Agda using coinductive data types. In CSP-Agda, CSP processes are in monadic form, which sup- ports a modular development of processes. In this paper, we implement two main models of CSP, trace and stable failures semantics, in CSP-Agda, and define the corresponding refinement and equal- ity relations. Because of the monadic setting, some adjustments need to be made. As an example, we prove commutativity of the external choice operator w.r.t. the trace semantics in CSP-Agda, and that refinement w.r.t. stable failures semantics is a partial order. All proofs and definitions have been type checked in Agda. Further proofs of algebraic laws will be available in the CSP-Agda repository.

==> eptcsdata.tex <==
\providecommand{\firstpage}{36}
\providecommand{\publicationstatus}{E. Komendantskaya and J. Power (Eds.):\\ Coalgebra, Horn Clause Logic Programming and Types\\
EPTCS 258, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.258.3}{10.4204/EPTCS.258.3}}
\pdfoutput=1

